Fine-grained activity recognition for assembly videos

In this paper we address the task of recognizing assembly actions as a structure (e.g. a piece of furniture or a toy block tower) is built up from a set of primitive objects. Recognizing the full range of assembly actions requires perception at a level of spatial detail that has not been attempted in the action recognition literature to date. We extend the fine-grained activity recognition setting to address the task of assembly action recognition in its full generality by unifying assembly actions and kinematic structures within a single framework. We use this framework to develop a general method for recognizing assembly actions from observation sequences, along with observation features that take advantage of a spatial assembly's special structure. Finally, we evaluate our method empirically on two application-driven data sources: (1) An IKEA furniture-assembly dataset, and (2) A block-building dataset. On the first, our system recognizes assembly actions with an average framewise accuracy of 70% and an average normalized edit distance of 10%. On the second, which requires fine-grained geometric reasoning to distinguish between assemblies, our system attains an average normalized edit distance of 23% -- a relative improvement of 69% over prior work.

==> leftovers.tex <==
% Enabled by large datasets collected from YouTube \cite{ucf101,kinetics,hmdb}
% and powerful neural classifiers,
% the field of action recognition has made impressive progress in ``web-scale" applications.
% Web-scale applications usually involve the classification of a very large set of short video clips (on the order of tens of seconds to a minute) drawn from a diverse set of high-level action categories---%
% for example, the benchmark dataset UCF101 contains classes like \texttt{playing guitar}, \texttt{playing piano}, \texttt{cutting in kitchen}, and \texttt{skydiving}.

% Web-scale activity recognition is an important task, and is critical for improving search and video retrieval tools.
% However, many applications of activity recognition require systems to understand videos in more detail.
% For instance, a system whose purpose is to automatically generate a recipe from a cooking video will need do distinguish between action categories defined at a finer level than \texttt{cutting in kitchen}---it needs to understand \emph{what} is being cut, and \emph{when}.
% Applications like this cooking example are now considered to be instances of \emph{fine-grained} action recognition.
% These settings usually involve longer, untrimmed videos in which a sequence of actions occurs. Additionally, there is usually less contextual information to make use of---videos share a common background, but actions are usually accompanied by the presence of certain objects.

% When a collaborative robot is working with a human partner to build
% a piece of furniture or an industrial part,
% the robot must be able to perceive which parts are connected and where,
% and it must be able to reason about how these connections can change as the result of its partner's actions.
% This need can also arise in industrial process monitoring and manufacturing applications,
% where an automated system verifies a product as it progresses through the assembly line.
% These assembly processes require systems that can reason geometrically \emph{and} temporally,
% relating the structure of an assembly to the manipulation actions that created it.

% \begin{figure}[htbp]
%     \centering
%     \input{diagrams/assembly-fsm.tex}
%     \caption{
%         A finite-state machine that accepts action sequences, and whose states are kinematic linkages.
%         This system represents all the assembly sequences that have the same
%         initial structure as the sequence in figure \ref{fig:assembly-seq},
%         and whose actions add or remove the blue and green square blocks.
%     }
%     \label{fig:assembly-fsm}
% \end{figure}

% Current approaches to activity recognition for assembly videos either focus on
% recognizing actions using an imperatively-defined, task-specific grammar,
% or estimating kinematic linkages without imposing constraints on which connectivity changes are acceptable.
% In this paper we describe a general method for recognizing assembly sequences
% that links action recognition and kinematic structure estimation
% using a weighted finite-state machine (WFSM).
% Our method has three main advantages.
% First, its process model applies to spatial assemblies in general,
% and can be composed with task-specific observation models easily and elegantly.
% Second, grounding its state in a kinematic linkage allows the machine
% to be constructed \emph{declaratively}---%
% we can obtain the set of viable successors for any state by computing the effect of a set of actions.
% Finally, the state's structure allows comparisons at multiple levels of granularity.
% Using analyses that range from a coarse-level measurement of which objects are common between two parts
% to the finest-grained assertion that two parts have exactly the same object, with exactly the same connections,
% in exactly the same poses, we can tell not only \emph{if} a prediction is wrong, but also \emph{where} it differs.

% Parsing videos of assembly is of great interest to the robotics and vision communities, evidenced by the existence of several works related to this task in three distinct subdisciplines: human-robot interaction, action recognition, and robotic perception.
% Multiple prior papers in the human-robot interaction literature use assembly parsers to enable applications such as collaborative or guided assembly  \cite{action-gupta-uist-2012, hadfield-blocks-iros-2018, robots-wang-hri-2020}. Since these applications require a system that works in real-time, solutions in this field are usually based on a combination of object tracking and greedy temporal parsing.
% Approaches to assembly parsing in action recognition have mostly been concerned with the broad task of defining a grammar on action sequences, and target assembly tasks along with other fine-grained activities (\eg cooking) in evaluations \cite{action-vo-cviu-2016, action-summers-iros-2012}.
% Alternatively, work in robotic perception has developed a rigorous probabilistic framework for the estimation the kinematic structure of an assembly, but has not focused on the task of temporal parsing \cite{kinem-models-sturm-ijcai-2009, kinem-models-martin-ijrr-2019, kinem-models-niekum-icra-2015}.
% In Section \ref{sec:related_work} we give a thorough description of these approaches.

% Despite the field's demonstrated interest in parsing assembly videos, to date there are no standardized frameworks or evaluations dedicated to this task.
% In this paper we present the first work addressing the specific task of assembly parsing, which we formulate as an extension of fine-grained activity recognition.
% We develop a conceptual framework that unifies previous approaches across domains and outlines the necessary components for assembly parsing systems.
% Improving over prior methods that defined grammars by hand for each application, our framework's novel sequence model applies to the class of assembly actions in general.
% % constructs a grammar over assembly actions given only a set available parts and their contact points, and supports parameter estimation from a training set in a straightforward way.
% % Finally, we present the first publicly-available multimodal (RGBD + IMU) dataset with fine-grained assembly labels, and compare assembly-parsing systems on this and two other datasets.
% Finally, we demonstrate assembly-parsing systems on two datasets in two separate application domains.

% \section{FINITE STATE MACHINES}
% \label{sec:fst_overview}
% %
% A finite state machine is a  convenient data structure
% that represents all sequences generated by a particular regular grammar,
% and which generalizes Hidden Markov models and linear-chain CRFs.
% Although there is a rich literature studying the application of finite state methods to sequence modeling problems in the speech and language processing communities,
% applications in activity recognition have not been as common.
% Therefore, we review the necessary concepts of finite-state methods
% before developing our model of assembly activities.
% For a more complete overview, we refer the reader to \cite{Mohri2008}

% A finite state acceptor (also FSA or just acceptor) is a directed graph whose edges are labeled with input symbols.
% Each vertex represents a state of the machine,
% and each edge represents the state transition induced by observing a particular symbol.
% If an edge is labeled with the special ``null" symbol $\epsilon$,
% the machine can transition along that edge without observing any symbol.
% An FSA is also marked with a set of valid initial states and a set of valid final states.
% If an acceptor contains a path from an initial state to a final state whose labels
% match some sequence of symbols,
% that sequence is valid under the machine's grammar
% (in other words, the machine accepts that sequence).
% In figure \ref{fig:assembly-fsm}, we illustrate an example finite state acceptor representing a simple grammar of assembly sequences.

% When an FSA's edges are augmented with a set of weights, it is called a weighted FSA (WFSA).
% The total weight of any path in a WFSA is defined to be the product of the weights on each edge in the path.
% If we define the weights of a WFSA to be state transition probabilities,
% then the machine implements a Markov chain defined on the states of the machine
% (although the resulting distribution on input sequences may not be Markov).

% Finally, an automaton that has been augmented to map input sequences to output sequences,
% rather than only accept a set of inputs,
% is called a weighted finite state transducer (WFST).
% The edges of a WFST are labeled with a triple defining the input symbol,
% the output symbol, and the weight associated with that input-output pair.
% In this case the machine can been seen as a discrete counterpart
% to the state-space dynamical systems common in signal processing, control, and robotics,
% since it maps an input sequence to an output sequence through a Markov-distributed latent state.
% Because any FSA can be implemented as an FST whose input labels are the same as its output labels,
% we will refer to state machines generically as FSTs for the remainder of this paper.

% Similarly to linear systems,
% two WFSTs can be composed so the output of one feeds into the input of the next.
% The two systems can be represented as a single WFST $T = T_1 \circ T_2$
% whose edge weights are given by
% %
% \begin{equation}
%     W_T(i, k) = \sum_j W_{T_1}(i, j) W_{T_2}(j, k)
% \end{equation}
% %
% Where $i$ ranges over the input of $T_1$, $j$ ranges over the output of $T_1$
% (equivalently, the input of $T_2$), and $k$ ranges over the output of $T_2$.
% For example, an observation model and a state transition model can be composed to
% form a hidden Markov model: $HMM = O \circ T$.

% When using finite state machines for sequence prediction tasks,
% one is usually concerned with finding an optimal path
% (\eg the most probable output sequence given a particular input sequence),
% or with finding the total weight of a set of paths
% (\eg the total probability of the data).
% These quantities can be computed using generalizations of the well-known Viterbi
% and Forward algorithms (respectively) for hidden Markov models or linear-chain CRFs.
%

% In the preceding section we identified the kinematic state of an assembly with the state of an FST,
% and we identified part addition or removal actions with the transducer's edge labels.
% In this section we will show how it can be used to predict assembly activities from video.
% Specifically, we construct an HMM for parsing assembly activities
% by composing our spatial assembly FST with an observation FST.

% The assembly FST serves as a process model, and is augmented with probabilistic edge weights
% %
% \begin{equation}
%     W_p(l, a, s \rightarrow s') = P(s' \mid s)
% \end{equation}
% %
% Where $W(l_i, l_o, s \rightarrow s')$ refers to the weight of an edge
% with input label $l_i$ and output label $l_o$
% that transitions from state $s$ to $s'$.

% We defer the definition of the input label $l$ because the structure of our framework allows us
% to define observation models in two different forms:
% we can either score \emph{actions} (corresponding to edges of the state machine),
% or we can score \emph{assemblies} (corresponding to states).
% Since an edge-weighted model reduces to a state-weighted one
% when observations depend only on the current state,
% these two decoding paradigms belong to the same general framework.
% Thus, the input label can either correspond to actions or to states.

% Given a video sequence $x_1, \ldots, x_T$,
% we construct an observation FST with a linear-chain structure.
% The input label of each edge is its sample index,
% its output corresponds to an action or a state,
% and its weights represent action detection probabilities:
% %
% \begin{equation}
%     W_o(t, l, s_t \rightarrow s_{t+1}) = P(x_t \mid l)
% \end{equation}

% The specific instantiation of the observation model can be chosen separately for each application.
% In section \ref{sec:experiments} we show two examples:
% one observation model is defined on detected hand locations and scores actions,
% and the other is defined on image pixels and scores states.

% To predict an action sequence from the video input,
% we compute the maximum-weight path in the composed transducer and read off the output labels.
% As mentioned in section \ref{sec:fst_overview}, this is analogous to the Viterbi algorithm
% and gives the maximum \emph{a posteriori} action sequence.

% \subsection{Toy airplane}
% \label{sec:airplanes}
% %
% In this section we show that a hand-annotated transition model from prior work can be implemented elegantly in our framework.
% Then, we show that our framework's ability to associate manipulation actions with their kinematic effects
% allows it to \emph{learn} that transition model from training sequences.

% We consider the toy airplane dataset of Vo and colleagues \cite{action-vo-cvpr-2014},
% which consists of 29 2--3 minute videos in which a person constructs one of three airplane models.
% There are 40 primitive parts and 12 distinct build sequences overall.

% Since this dataset was created to test methods for compositional action recognition,
% its labeling scheme and prior evaluation conventions do not describe the full variability of assembly---%
% in particular there are no mistakes and no backtracks.
% In terms of our framework, every action in this dataset is a connection
% and every object is placed in its correct location with respect to the final model.
% Thus for this dataset, an action can be identified by recognizing only the object that is added to the model
% (recall that a general assembly scenario requires us to define
% not only \emph{what} will be added, but also \emph{where}).
% This reduces the task of parsing a sequence of assembly states to
% identifying which objects were added to the model, and in what order.

% \begin{figure*}[htbp]
%     \centering
%     \input{diagrams/airplane-state-machine.tex}
%     \caption{
%         State machine generating the build sequences of the toy airplane dataset
%         (reproduced from \cite{action-vo-cvpr-2014}).
%         Each box represents a sub-part of the model.
%         For example, Body(4) means the Body sub-part is assembled from 4 primitive objects.
%     }
%     \label{fig:airplane-sm}
% \end{figure*}

% The videos of this toy airplane dataset are additionally constrained to conform to a set of pre-specified AND-OR rules---for example, $\texttt{wheel} \rightarrow \texttt{wheel}_1 \cap \texttt{wheel}_2$.
% In figure \ref{fig:airplane-sm}, we reproduce the original state machine from \cite{action-vo-cvpr-2014} summarizing these AND-OR rules.
% Notice that this machine does not accept every assembly sequence that results in a valid airplane model---%
% only sequences in which the model is built in sub-parts, in a particular order.
% For example, it cannot recognize an assembly sequence in which someone builds the body,
% then builds part of the nose, then builds the tail, and finally comes back to finish the nose.

% Because of these simplifications,
% the grammar of Vo and colleagues can be represented as a subset of ours.
% In Figure \ref{fig:airplane-part-sm} we illustrate three examples of their hierarchical AND-OR rules, 
% implemented as FSTs in our framework.

% %
% \begin{figure*}[htbp]
%     \centering
%     \input{diagrams/airplane-state-machine-3.tex}
%     \input{diagrams/airplane-state-machine-2.tex}
%     \input{diagrams/airplane-state-machine-1.tex}
%     \caption{
%         An equivalent state machine to the one in in
%         Figure \ref{fig:airplane-sm},
%         represented as a composition of FSTs implementing the AND-OR rules of Vo and colleagues.
%         TOP: High-level rule mapping semantic parts to completed airplane models.
%         CENTER: Expansion of a mid-level transducer, which maps a sequence of semantic parts to a mid-level part---in this case, a nose-wing-tail (NWT) combination.
%         BOTTOM: The lowest-level transducer, mapping a sequence of primitive objects to a semantic part.
%     }
%     \label{fig:airplane-part-sm}
% \end{figure*}

% \subsection{Toy airplane videos}
% \label{sec:experiments_airplane}
% %
% Next, we use our framework to decode spatial assemblies
% \emph{without constructing by hand the explicit state machine shown in Fig. \ref{fig:airplane-sm}}.
% Instead, we use the actions labeled in our training set and our model of spatial assembly sequences
% to \emph{learn} a state machine.

% \subsubsection{Experimental Setup}
% \label{sec:experiments_airplane_setup}
% %
% In our experiments we perform leave-one-out cross-validation;
% thus each fold has 28 training videos and 1 test video.

% Our model uses observation scores taken directly from the Sequential Interval Network \cite{action-vo-cvpr-2014}, whose code has been made available online.
% This approach scores actions (corresponding to part reaches)
% by determining when the hand is near one of the five bins containing the model's components.
% If a reach is detected, each part-reach action is assigned a Gaussian probability
% proportional to the hand's distance from the bin containing that part.
% If not, all part-reach actions are assigned a constant, baseline value.
% We additionally pre-process the input sequence by segmenting it according to part-reach detections.
% We take the average action scores within segments, and ignore the scores outside segments.

% When training the model,
% we compute the initial and final states' weights,
% along with the edge weights of state transitions,
% using frequencies observed in the training set.
% We also tie some states in our grammar to match the logic of Figure \ref{fig:airplane-sm}---
% although by default a build sequence in which wheels were added to the model
% is different from one in which they were not,
% the original grammar considers these sequences to be equivalent.
% We can implement this notion neatly by checking whether states are equivalent up to the wheel parts:
% \ie $s \sim s'$ if $ (s / s') \cup (s' / s) \subseteq \{ \texttt{wheel}_1, \texttt{wheel}_2\}$.
% The Gaussian means and covariances of the Sequential Interval Network's observation model
% are also estimated during the training process as described in \cite{action-vo-cvpr-2014}.

% \subsubsection{Results}
% \label{sec:experiments_airplane_results}

% To compare with prior work,
% we report the average task classification accuracy.
% This is the proportion of times the model identified a build sequence
% as belonging to the correct airplane model
% (recall that the dataset consists of build sequences corresponding to three different
% types of airplanes).
% Our method achieves 83\% classification accuracy,
% while the Sequential Interval Network performs at 96\%.
% The discrepancy between methods is due to the noisy hand detections supplied with this dataset.
% This leads to missed-detection and false-alarm errors in the reach detection stream,
% resulting in input sequences that deviate from the models' grammars.
% The Sequential Interval Network overcomes this issue by averaging over all possible segmentations
% of the input sequence, resulting in an algorithm whose runtime complexity
% is \emph{quadratic} in the number of \emph{samples} in the sequence.
% On the other hand, our implementation is slightly less robust
% but enjoys a runtime complexity that is \emph{linear} in the number of \emph{segments},
% and our grammar is not tied to any single implementation.

General:
\begin{align}
    \Prob{s, y} &= \prod_{m=1}^{M} \prod_{t=b_m}^{b_m + d_m}
        \CondProb{I_t}{x_t, s_m, s_{m-1}}
        \CondProb{x_t}{x_{t-1}, s_m} \\
        & \CondProb{d_m}{s_m, s_{m-1}}
        \CondProb{s_m}{s_{m-1}}
\end{align}

$y_t \coloneqq (I_t, x_t)$

In this case,
$
    \CondProb{I_t}{x_t, s_m, s_{m-1}}
    \CondProb{x_t}{x_{t-1}, s_m} =
    \CondProb{y_t}{y_{t-1}, s_m, s_{m-1}}
$

If the time dependence in the pose sequence can be ignored
(for instance, if poses have already been estimated),
then we obtain a standard Markov-style observation:
$
    \CondProb{y_t}{s_m, s_{m-1}} = \CondProb{y_t}{s_m, s_{m-1}}
$

\begin{align}
    \Prob{s, y} &= \prod_{m=1}^{M} \prod_{t=b_m}^{b_m + d_m}
        \CondProb{y_t}{s_m, s_{m-1}} \\
        & \CondProb{d_m}{s_m, s_{m-1}}
        \CondProb{s_m}{s_{m-1}}
\end{align}

If segments are known:
\begin{align}
    \Prob{s, y} &= \prod_{m=1}^{M}
        \CondProb{y_m}{s_m, s_{m-1}} \CondProb{s_m}{s_{m-1}}
\end{align}


==> tables/results-table-airplane.tex <==
\renewcommand{\arraystretch}{1.5}
\pgfplotstabletypeset[
    col sep=comma,
    columns={[index]0,[index]1,[index]2},
    columns/0/.style={string type, column type=r, column name={ } },
    columns/theirs/.style={string type, column type=r, column name={ Vo \emph{et al.}} },
    every head row/.style={before row=\toprule,after row=\midrule},
    every last row/.style={after row=\bottomrule},
    every row 0 column theirs/.style={string type, column type=r}
    %every row 1 column rgb+depth/.style={postproc cell content/.style={@cell content=\underline{##1}}},
    %every row 2 column rgb+depth/.style={postproc cell content/.style={@cell content=\textbf{##1}}},
    %every row 3 column rgb+depth/.style={postproc cell content/.style={@cell content=\underline{##1}}},
    %every row 4 column rgb+depth/.style={postproc cell content/.style={@cell content=\textbf{##1}}},
    %every row 5 column rgb+depth/.style={postproc cell content/.style={@cell content=\underline{##1}}},
    %every row 6 column rgb+depth/.style={postproc cell content/.style={@cell content=\textbf{##1}}},
    %every row 7 column rgb+depth/.style={postproc cell content/.style={@cell content=\textbf{##1}}},
    %every row 8 column rgb+depth/.style={postproc cell content/.style={@cell content=\textbf{##1}}},
    %every row 9 column rgb+depth/.style={postproc cell content/.style={@cell content=\underline{##1}}},
    %every row 10 column rgb+depth/.style={postproc cell content/.style={@cell content=\textbf{##1}}},
    %every row 11 column rgb+depth/.style={postproc cell content/.style={@cell content=\textbf{##1}}},
]{tables/airplane-results.csv}

==> tables/results-table-connections.tex <==
\renewcommand{\arraystretch}{1.5}
\pgfplotstabletypeset[
    col sep=comma,
    columns/name/.style={string type, column type=r, column name={ } },
    every head row/.style={before row=\toprule,after row=\midrule},
    every last row/.style={after row=\bottomrule},
    every column/.style={string type, string replace*={+/-}{$\pm$}}
]{tables/connections-results.csv}
